Focus Is What You Need For Chinese Grammatical Error Correction

Chinese Grammatical Error Correction (CGEC) aims to automatically detect and correct grammatical errors contained in Chinese text. In the long term, researchers regard CGEC as a task with a certain degree of uncertainty, that is, an ungrammatical sentence may often have multiple references. However, we argue that even though this is a very reasonable hypothesis, it is too harsh for the intelligence of the mainstream models in this era. In this paper, we first discover that multiple references do not actually bring positive gains to model training. On the contrary, it is beneficial to the CGEC model if the model can pay attention to small but essential data during the training process. Furthermore, we propose a simple yet effective training strategy called OneTarget to improve the focus ability of the CGEC models and thus improve the CGEC performance. Extensive experiments and detailed analyses demonstrate the correctness of our discovery and the effectiveness of our proposed method.

==> One Target GEC/tables/exp1.tex <==
\begin{table}[!tbp]
\centering
\scalebox{0.8}{
\begin{tabular}{l|l|ccc|ccc}
\toprule
\multicolumn{2}{c|}{\multirow{2}{*}{\textbf{Strategy}}} & \multicolumn{3}{c|}{Seq2Seq} & \multicolumn{3}{c}{Seq2Edit} \\
\multicolumn{2}{c|}{} & \textbf{P} & \textbf{R} & \textbf{F}$_{0.5}$ & \textbf{P} & \textbf{R} & \textbf{F}$_{0.5}$ \\ 
\midrule
\multirow{8}{*}{\MethodName{}} & \textbf{lev\_sim} & 46.14 & 27.30 & \textbf{40.55} & \textbf{47.20} & 16.60 & \textbf{34.48} \\
& \textbf{lev\_dis} & 43.72 & 27.96 & 39.29 & 38.38 & 18.34 & 31.50 \\ 
\cmidrule{2-8}
& \textbf{jac\_sim} & 46.25 & 26.71 & \textbf{40.35} & 45.75 & 15.63 & 33.02 \\
& \textbf{jac\_dis} & 43.68 & 26.33 & 38.59 & 38.77 & 17.73 & 31.34 \\ 
\cmidrule{2-8}
& \textbf{edi\_least} & \textbf{46.33} & 24.69 & 39.42 & 43.90 & 16.30 & 32.80 \\
& \textbf{edi\_most}  & 44.04 & 27.18 & 39.18 & 37.25 & \textbf{21.21} & 32.25 \\ 
\cmidrule{2-8}
& \textbf{random} & 45.45 & 25.44 & 39.27 & 41.42 & 17.27 & 32.37 \\
\midrule
\multicolumn{2}{c|}{\textbf{full}} & 44.08 & \textbf{28.16} & 39.60 & 41.36 & 19.18 & 33.59 \\ 
\bottomrule
\end{tabular}}
\caption{Performance on MuCGEC-dev of Seq2Seq-based and Seq2Edit-based models with different strategies.}
\label{tab:exp1}\end{table}

==> One Target GEC/tables/exp2.tex <==
\begin{table}[!htpb]
\centering
\scalebox{0.8}{
\begin{tabular}{llccc}
\toprule
\textbf{Dataset} & \textbf{\#sample} & \textbf{P} & \textbf{R} & \textbf{F$_{0.5}$} \\ 
\hline
1-target & 127,986 & \textbf{42.03} & 15.67 & \textbf{31.45} \\ 
2-target & 255,972 & 37.50 & \textbf{18.51} & 31.11 \\
3-target & 383,958 & 39.22 & 16.74 & 30.92 \\ 
\bottomrule
\end{tabular}}
\caption{Performance on MuCGEC-dev of GECToR models trained with 1$\sim$3-target datasets respectively. For the sake of simplicity, we do not introduce pre-training on synthetic parallel dataset and multi-stage fine-tuning as Omelianchunk \textit{et al.} \cite{omelianchuk-etal-2020-gector}.}
\label{tab:exp2}
\end{table}


==> One Target GEC/tables/intro.tex <==
\begin{table}[t]
\centering
\small
\renewcommand\arraystretch{1.2}
\begin{tabular}{ll}
\hline
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Source}}} & 我能胜任这此职务  \\
\multicolumn{1}{c}{} & I am competent for this the position. \\ 
\hline
\multirow{2}{*}{\textbf{Ref. 1}} & 我能胜任\textcolor{red}{这\sout{此}}职务。 \\
& I am competent for \textcolor{red}{this \sout{the}} position. \\
\multirow{2}{*}{\textbf{Ref. 2}} & 我能胜任\textcolor{red}{\sout{这}此}职务。 \\
& I am competent for \textcolor{red}{\sout{this} the} position.  \\ 
\hline
\end{tabular}
\caption{The example of CGEC. The \textcolor{red}{correction part} is marked.}
\label{tab:intro}
\end{table}

==> One Target GEC/tables/lang8_statistics.tex <==
\begin{center}
\begin{table*}[!htb]
\centering
\scalebox{0.8}{
\begin{tabular}{lccccc}
\toprule
\textbf{\# target} & \textbf{\# source (perc.)} & \textbf{length} & \textbf{mean of Levenshtein ratio} & \textbf{variance of Levenshtein ratio} & \textbf{\# edits/target}\\ 
\hline
1 & 290,493 (49.99\%) & 18.8 & 0.84 & 0.0185 & 2.1 \\
2 & 168,044 (28.92\%) & 20.1 & 0.83 & 0.0196 & 2.5 \\
3 &  73,196 (12.60\%) & 20.8 & 0.81 & 0.0202 & 2.7 \\
4 &  28,817 (4.96\%) & 21.5 & 0.81 & 0.0207 & 2.9 \\
5 &  11,507 (1.98\%) & 22.0 & 0.80 & 0.0213 & 3.0 \\
6 &   4,853 (0.84\%) & 22.3 & 0.80 & 0.0211 & 3.1 \\
7 &   2,155 (0.37\%) & 23.1 & 0.79 & 0.0216 & 3.2 \\
\textgreater 8  &  2,020 (0.35\%) & 22.7 & 0.78 & 0.0244 & 3.3 \\
\hline 
\textbf{Total} & 581,085 (100.00\%) & 19.7 & 0.82 & 0.0201 & 2.5 \\[-3pt]
\bottomrule
\end{tabular}}
\caption{Data statistics of Lang8 dataset, including the number (proportion) of unique ungrammatical source sentences (i.e., grammatical source sentences have been removed) with different number of corrected target sentences, the average length per source sentence, the average Levenshtein ratio between source sentences and corresponding target sentences, the variance of Levenshtein ratio and the average number of edits per target sentence.}
\label{tab:lang8_statistics}
\end{table*}
\end{center}

==> One Target GEC/tables/mucgec_test.tex <==
\begin{table}[!tbp]
\centering
\scalebox{0.8}{
\begin{tabular}{l|ccc|ccc}
\toprule
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{}}} & \multicolumn{3}{c|}{Seq2Seq} & \multicolumn{3}{c}{Seq2Edit} \\
\multicolumn{1}{c|}{} & \textbf{P} & \textbf{R} & \textbf{F}$_{0.5}$ & \textbf{P} & \textbf{R} & \textbf{F}$_{0.5}$ \\ 
\midrule
\textbf{Zhang et al.} \cite{zhang-etal-2022-mucgec} & 43.81 & 28.56 & 39.58 & 44.11 & 27.18 & 39.22 \\
\textbf{Zhang et al.} $\clubsuit$ & 46.49 & 28.64 & \textbf{41.34} & 46.62 & 25.60 & 40.04 \\
\midrule
\textbf{lev\_sim} & 45.95 & 28.87 & 41.09 & 47.34 & 25.97 & \textbf{40.65} \\
\textbf{random} & 47.14 & 27.28 & 41.15 & 44.66 & 27.55 & 39.73 \\ 
\bottomrule
\end{tabular}}
\caption{Comparison of our single models with related work on MuCGEC-test. We only report part of the results due to the limitation of space. Models in the first block are trained using the full dataset (with 1,557,438 paired samples) and models in the second block are trained using one-target dataset (with 1,056,600 paired samples). The symbol of “$\clubsuit$” means the results of our re-implemented baseline method.}
\label{tab:mucgec_test}\end{table}

==> One Target GEC/tables/overall_statistics.tex <==
\begin{table*}[!htb]
\centering
\scalebox{0.9}{
\begin{tabular}{lccccc}
\toprule
\textbf{Dataset} & \textbf{\# sample} & \textbf{\# err. sample (perc.)} & \textbf{\# unique source (perc.)} & \textbf{length} & \textbf{Levenshtein ratio} \\ 
\hline
Lang8 & 1,220,906 & 1,096,387 (89.8\%) & 695,275 (56.95\%) & 18.9 & 0.84 \\
HSK & 156,870 & 96,049 (61,23\%) & 156,358 (99.67\%) & 27.3 & 0.95 \\ 
MuCGEC-dev & 2,467 & 2,412 (97.77\%) & 1,137 (46.09\%) & 44.0 & 0.90 \\
\bottomrule
\end{tabular}}
\caption{Data statistics of Lang8, HSK and MuCGEC-dev, including the number of paired samples, the number (proportion) of erroneous samples, the number (proportion) of unique source sentences, the average length per source sentence and the average Levenshtein ratio between source sentences and corresponding target sentences.}
\label{tab:overall_statistics}
\end{table*}
